Probabilistic Hierarchical Forecasting with Deep Poisson Mixtures

Hierarchical forecasting problems arise when time series have a natural group structure, and predictions at multiple levels of aggregation and disaggregation across the groups are needed. In such problems, it is often desired to satisfy the aggregation constraints in a given hierarchy, referred to as hierarchical coherence in the literature. Maintaining coherence while producing accurate forecasts can be a challenging problem, especially in the case of probabilistic forecasting. We present a novel method capable of accurate and coherent probabilistic forecasts for time series when reliable hierarchical information is present. We call it Deep Poisson Mixture Network (DPMN). It relies on the combination of neural networks and a statistical model for the joint distribution of the hierarchical multivariate time series structure. By construction, the model guarantees hierarchical coherence and provides simple rules for aggregation and disaggregation of the predictive distributions. We perform an extensive empirical evaluation comparing the DPMN to other state-of-the-art methods which produce hierarchically coherent probabilistic forecasts on multiple public datasets. Comparing to existing coherent probabilistic models, we obtain a relative improvement in the overall Continuous Ranked Probability Score (CRPS) of 11.8% on Australian domestic tourism data, and 8.1% on the Favorita grocery sales dataset, where time series are grouped with geographical hierarchies or travel intent hierarchies. For San Francisco Bay Area highway traffic, where the series' hierarchical structure is randomly assigned, and their correlations are less informative, our method does not show significant performance differences over statistical baselines.

==> iclr/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/section1_introduction_raw.tex <==
%\subsection{Problem Formulation}
There are several cases where forecast users need simultaneous forecasts throughout a hierarchy or group structure. For example, demand forecast in retail and e-commerce requires aggregation across products \citep{seeger2017hierarchical_retail2} and geographies and electricity load forecasting requires predictions to be aggregated at different regional levels. \citep{taieb2019hierarchical_regularized_regression, jeon2019hierarchical_regional_wind_electricity}. In those cases, coherence is satisfied when the forecast of disaggregated series adds-up to the forecast of aggregated series.

The main goal of hierarchical forecasting is to produce coherent forecasts by leveraging available information across all the levels of the structure. Prior solutions to the challenge depended on two-stage approaches where \emph{base forecasts} were created and later reconciled. More recent work extended the generation of probabilistic hierarchical forecasts into single and simplified models \NM{Add citations here?}. Some limitations that we find in current solutions are (i) their efficiency, as any new hierarchical structure of interest would require to fit a whole new model \NM{This is not clear. Do you mean that complex hierarchies will be compute resource limited? or do you mean generalizing to additional levels not present in the original data is harder?}, (ii) their accuracy, as the models tend to use restrictive probabilistic models, to enable reconciliation. \NM{Need to elaborate on this. Explicitly mention assumption about normal distribution etc.}

\begin{enumerate}%[(i)]
    \item \textbf{Limited Research on Probabilistic Forecasts}: \KO{Paraphrase }

    \item \textbf{Restrictive Distributional Assumptions}:
    
    
    \item \textbf{Efficiency}: Finally, the \PMM \ can accommodate unrevealed hierarchical structures during its optimization. Its aggregation and disaggregation rules also allow users to easily generate any new marginal distribution. In contrast, other more complex approaches require the hierarchical structure in advance, and changes to the structure need to fit a whole new specialized model.
\end{enumerate}

%\subsection{Motivation}
\NM{High level comment for this section. This seems too detailed without introducing PMMs formally. Can we keep it simple by focusing on the fact that we produce flexible joint distributions with simple aggregation/disaggregation rules, and works well with a neural network?}
In this work we explore the Poisson Mixture Mesh Convolutional Neural Network (\ours) solution for the probabilistic hierarchical forecasting challenge, as we envision that its following characteristics can help to tackle the mentioned limitations:

\begin{enumerate}%[(i)]
    \item \textbf{Probabilistic Coherence}: The Poisson Mixture Mesh (\PMM) defines a joint distribution across all levels of the time series structures. By construction, it guarantees probabilistic coherence of its predictions, with its simple aggregation and disaggregation rules.

    \item \textbf{Enhanced Accuracy} \NM{Accuracy improvement is not automatically guaranteed. We should focus on the flexibility}: The \PMM \ is a flexible and powerful improvement over available hierarchical methods capable of producing coherent, probabilistic forecasts that rely on strong assumptions on the distributions, like Gaussian noise, that enable its reconciliation strategies. Additionally, the \PMM \ representation is independent of the model that supports and can leverage the rich literature on neural forecasting models.
    
    \item \textbf{Efficiency}: Finally, the \PMM \ can accommodate unrevealed hierarchical structures during its optimization. Its aggregation and disaggregation rules also allow users to easily generate any new marginal distribution. In contrast, other more complex approaches require the hierarchical structure in advance, and changes to the structure need to fit a whole new specialized model.
\end{enumerate}

The paper is structured as follows. Section \ref{section:literature} introduces notation and reviews relevant literature on hierarchical forecasting. Sections~\ref{section:pmm} and \ref{section:pmmcnn} describe our methodology. In Section \ref{section:experiments} we provide an empirical evaluation on real world hierarchical data, where we showcase the advantages of our method. Finally, in Sections~\ref{section:conclusion} we discuss future work and conclude.


==> sections/section3_pmm.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=100mm]{images/pmm_sample.pdf}
\caption{The Poisson Mixture distribution has desirable properties that make it well-suited for probabilistic hierarchical forecasting for count data. 
Under minimal conditions, its aggregation rule implies probabilistic coherence of the random variables it models.
}
\label{fig:poisson_mixture}
\end{figure}
%

\subsection{Joint Poisson Mixture Distribution}

We start by postulating that the forecast joint distribution of bottom level future multivariate time series $\mathbf{y}_{[b][t+1:t+h]} \in \mathbb{N}^{N_{b} \times h}$ is captured by \EDIT{ the following mixture:
\begin{eqnarray}
\label{eq:general_mixture}
    \mathrm{P}\left(\mathbf{y}_{[b][t+1:t+h]}\right) &=& 
    \int (\; \mathrm{P}(\blambda_{[b][t+1:t+h]}) \; \mathrm{P}(\mathbf{y}_{[b][t+1:t+h]} \vert \blambda_{[b][t+1:t+h]}) \;) \; d\blambda_{[b][t+1:t+h]} \\
    &=& 
	\int (\;
	\mathrm{P}(\blambda_{[b][t+1:t+h]})
	\prod_{(\beta,\tau) \in [b][t+1:t+h]} \mathrm{Poisson}(y_{\beta,\tau} \vert \lambda_{\beta,\tau}) \;) \; d\blambda_{[b][t+1:t+h]} 
\end{eqnarray}
Equation~(\ref{eq:general_mixture}) is a standard Bayesian formulation. We introduce latent multi-variate Poisson rates $\blambda_{[b][t+1:t+h]}$ described by the joint distribution $\mathrm{P}(\blambda_{[b][t+1:t+h]})$, and conditioned on the rates the target variables $\mathbf{y}_{[b][t+1:t+h]}$ are described by independent Poisson distributions
%Equation \eqref{eq:general_mixture} assumes that observations are conditionally independent given the Poisson rates 
%In order to make the joint distribution from Equation~(\ref{eq:general_mixture}) compatible with neural networks, we rely on two simplifying assumptions. First, the observations are assumed to be \emph{conditionally independent} given the Poisson rates, namely
% \begin{eqnarray}
% \label{eq:conditional_indep}
%     y_{\beta,\tau} | \lambda_{\beta,\tau} & \indep & y_{\beta',\tau'} | \lambda_{\beta',\tau'} \\
%     \mathrm{P}(y_{\beta,\tau},  y_{\beta',\tau'} \vert \lambda_{\beta,\tau}, \lambda_{\beta',\tau'}) &=&  \mathrm{P}(y_{\beta,\tau} \vert \lambda_{\beta,\tau}) \mathrm{P}( y_{\beta',\tau'} \vert \lambda_{\beta',\tau'})
% \end{eqnarray} 
\EDITtwo{
\begin{align}
\label{eq:conditional_indep}
\begin{split}
    %y_{\beta,\tau} | \lambda_{\beta,\tau} \indep y_{\beta',\tau'} | \lambda_{\beta',\tau'} \qquad\qquad\quad\quad\;\\
    \mathrm{P}(y_{\beta,\tau},  y_{\beta',\tau'} \vert \lambda_{\beta,\tau}, \lambda_{\beta',\tau'}) =  \mathrm{P}(y_{\beta,\tau} \vert \lambda_{\beta,\tau}) \mathrm{P}( y_{\beta',\tau'} \vert \lambda_{\beta',\tau'})    
\end{split}
\end{align}
}

for all $ (\beta, \tau) \neq (\beta',\tau') \text{ and } (\beta, \tau), (\beta', \tau') \in [b][t+1:t+h]$, and 

\begin{equation}
    \mathrm{P}(y_{\beta,\tau} \vert \lambda_{\beta,\tau}) = \mathrm{Poisson}(y_{\beta,\tau} \vert \lambda_{\beta,\tau}) = \frac{\lambda_{\beta,\tau}^{y_{\beta,\tau}}}{y_{\beta,\tau}!} e^{-\lambda_{\beta,\tau}}
\end{equation}

All interesting correlations in the model are captured through the joint distribution of the latent variables, and our goal is to estimate the joint distribution $\mathrm{P}(\blambda_{[b][t+1:t+h]})$ which describes the data best. Since we are interested in unconditional distribution of $\mathbf{y}_{[b][t+1:t+h]}$, we integrate out the latent Poisson variables in Equation~(\ref{eq:general_mixture}). 

One of the key innovations of our work is to approximate the joint distribution of Poisson rates by a finite set of weighted multivariate samples 
}

%all dependencies in the observations are captured by the joint distribution of the Poisson rates $\blambda_{[b][t+1:t+h]}$. The setup so far is similar to a standard Bayesian hierarchical formulation. However, instead of assuming a parametric model like Gaussian process that drives the latent variables, with the \ours\; we approximate the joint distribution of the Poisson rates by a finite mixture of weighted multi-variate samples %\KO{Missing $[k]$ indices in Equation~(\ref{eq:finite_mixture})?, or intro to $[k]$?}\RM{Changed $N_\lambda$ to $N_k$ and $k\to\kappa$ throughout the paper, for consistency in notations that $|[k]|=N_k$.}
%\vspace{5mm}
%Second, we approximate the joint distribution of Poisson rate components\footnote{This Poisson rate joint distribution, models the transition between latent mixture variables and is fundamental for the aggregation rule and covariance structure.} with the following finite mixture of weighted multi-variate samples:
\begin{align} \label{eq:finite_mixture}
    \mathrm{P}(\blambda_{[b][t+1:t+h]}) = \sum_{\kappa=1}^{N_k} w_\kappa \prod_{(\beta,\tau) \in [b][t+1:t+h]} \delta(\lambda_{\beta, \tau} - \lambda_{\beta, \kappa, \tau})
\end{align}
where $\delta(x)$ is the Dirac Delta function. The Poisson rates $\blambda_{[b][k][t+1:t+h]} \in \mathbb{R}^{N_{b} \times N_{k} \times h}$ and the associated weights $\mathbf{w}_{[k]} \in \mathbb{R}^{N_{k}}$, with $\mathbf{w}_{[k]} \geq 0$ and $\sum_{\kappa=1}^{N_k}w_\kappa = 1$,  are parameters of the probability distribution to be estimated. The number of Poisson components $\mid[k]\mid = N_k$ is a hyperparameter of the model that controls the fidelity of the mixture distribution. \EDIT{ The finite mixture representation is a flexible non-parametric formulation of the joint distribution and allows us to lean heavily on the strength of neural networks to learn non-parametric functions.

%Under the \textit{conditional independence} and \textit{unmixing property} 
Substituting Equation~(\ref{eq:finite_mixture}) into Equation~(\ref{eq:general_mixture}), we get the final form of the joint distribution for bottom level time series} $\mathbf{y}_{[b][t+1:t+h]}$ in \ours\,
\begin{align} \label{eq:joint_distribution}
    \mathrm{P}\left(\mathbf{y}_{[b][t+1:t+h]}\right) &= \sum_{\kappa=1}^{N_{k}} w_\kappa \prod_{(\beta,\tau) \in [b][t+1:t+h]}  \mathrm{Poisson}(y_{\beta,\tau} \vert \lambda_{\beta,\kappa,\tau})
    %\\
    %&= \sum_{\kappa=1}^{N_{k}} w_\kappa \prod_{(\beta,\tau) \in [b][t+1:t+h]}\left( \frac{(\lambda_{\beta,\kappa,\tau})^{^{y_{\beta,\tau}}}\exp{\{-\lambda_{\beta,\kappa,\tau}\}}}{(y_{\beta,\tau})!}\right) 
    %&= \mathrm{PM}[\mathbf{w}_{[k]}, \blambda_{[b][k][t+1:t+h]}]
\end{align}

%This is a flexible class of distributions and is generally suited for count data. %MF: I removed this comment as we didn't mention `count data' anywhere in prior.
The final distribution can also be interpreted as a multivariate kernel density approximation, with Poisson kernels, to the actual probability distribution. We show an example of the Poisson mixture distribution in Figure~\ref{fig:poisson_mixture}.

%The mixture first determines a latent categorical variable $K$ that selects a state, and conditional on the selection, an independent Poisson random variable that determines the observations. Using weights $\mathbf{w}_{[k]} \in \mathbb{R}^{N_{\lambda}}$ and rates 
%$\blambda_{[b][k][t+1:t+h]} \in \mathbb{R}^{N_{b}\times N_{\lambda} \times h}$ the full joint likelihood can be parametrized as:
% \begin{equation}
% \label{eq:pmm_joint}
% \begin{aligned}
% 	\mathrm{P}\left(\mathbf{y}_{[b][:t+h]}\right) 
%     &=
% 	\sum_{k=1}^{N_{\lambda}} \mathrm{P}(K=k) \mathrm{P}\left(\mathbf{y}_{[b][:t+h]}\,|\,K=k\right) 
% 	=\sum_{k=1}^{N_{\lambda}} w_k \prod_{(b,t) \in [b][:t+h]}\left( \frac{(\lambda_{b,k,t})^{^{y_{b,t}}}\exp{\RM{\{-\lambda_{b,k,t}\}}}}{(y_{b,t})!}\right)
% \end{aligned}
% \end{equation}
%\begin{equation}
%\label{eq:pmm_joint}
%\begin{aligned}
%	\mathrm{P}\left(\mathbf{y}_{[b][t+1:t+h]}\right) 
%    &=
%	\sum_{k=1}^{N_{\lambda}} \mathrm{P}(K=k) \mathrm{P}\left(\mathbf{y}_{[b][t+1:t+h]}\,|\,K=k\right) \\
%	&=\sum_{k=1}^{N_{\lambda}} w_k \prod_{(\beta,\tau) \in [b][t+1:t+h]}\left( %\frac{(\lambda_{\beta,k,\tau})^{^{y_{\beta,\tau}}}\exp{\{-\lambda_{\beta,k,\tau}\}}}{(y_{\beta,\tau})!}\right)
%\end{aligned}
%\end{equation}


% we denote such Poisson Mixture distributed variable as
%We describe properties of the Poisson Mixture distribution that make it exceptionally suited for the hierarchical forecasting task below.
\subsection{Marginal Distributions for Bottom Series}\label{sec:bottom_marginal_distribution}
Equation~(\ref{eq:joint_distribution}) describes the joint distribution of all bottom level time series.
We can derive the marginal distribution for one of the bottom level series $\beta \in [b]$ and for a single future time period $\tau \in [t+1:t+h]$ by integrating out the remaining time and series indices. The marginal distribution is:
% \begin{eqnarray}
%     \mathrm{P}(y_{\beta, \tau}) &=& \sum_{\mathbf{y}_{[b][t+1:t+h] \setminus (\beta, \tau)}} \sum_{\kappa=1}^{N_{k}} w_\kappa \prod_{(\beta^\prime,\tau^\prime) \in [b][t+1:t+h]}\mathrm{Poisson}(y_{\beta^\prime,\tau^\prime} \vert \lambda_{\beta^\prime,\kappa,\tau^\prime}) \nonumber \\
%                                 &=& \sum_{\kappa=1}^{N_{k}} w_\kappa \; \mathrm{Poisson}(y_{\beta,\tau} \vert \lambda_{\beta,\kappa,\tau}) \times \nonumber \\ 
%                                 && \quad \prod_{(\beta^\prime,\tau^\prime) \in [b][t+1:t+h] \setminus (\beta, \tau)} \quad \sum_{y_{\beta^\prime,\tau^\prime}}\mathrm{Poisson}(y_{\beta^\prime,\tau^\prime} \vert \lambda_{\beta^\prime,\kappa,\tau^\prime}) \nonumber \\
%                                 &=& \sum_{\kappa=1}^{N_k} w_\kappa \; \mathrm{Poisson}(y_{\beta,\tau} \vert \lambda_{\beta,\kappa,\tau})
% \end{eqnarray}
\begin{align}
    \mathrm{P}(y_{\beta, \tau}) 
    &= \sum_{\mathbf{y}_{[b][t+1:t+h] \setminus (\beta, \tau)}} \sum_{\kappa=1}^{N_{k}} w_\kappa \prod_{(\beta^\prime,\tau^\prime) \in [b][t+1:t+h]}\mathrm{Poisson}(y_{\beta^\prime,\tau^\prime} \vert \lambda_{\beta^\prime,\kappa,\tau^\prime}) \nonumber \\
    &= \sum_{\kappa=1}^{N_{k}} w_\kappa \; \mathrm{Poisson}(y_{\beta,\tau} \vert \lambda_{\beta,\kappa,\tau}) \times \nonumber \prod_{(\beta^\prime,\tau^\prime) \in [b][t+1:t+h] \setminus (\beta, \tau)} \quad \sum_{y_{\beta^\prime,\tau^\prime}}\mathrm{Poisson}(y_{\beta^\prime,\tau^\prime} \vert \lambda_{\beta^\prime,\kappa,\tau^\prime}) \nonumber \\
    &= \sum_{\kappa=1}^{N_k} w_\kappa \; \mathrm{Poisson}(y_{\beta,\tau} \vert \lambda_{\beta,\kappa,\tau})
\end{align}

\EDIT{ We get a clean final expression for the marginal distribution}, which is equivalent to simply dropping all other time series and time periods from the product in Equation~(\ref{eq:joint_distribution}).

\subsection{Marginal Distributions for Aggregate Series}
\label{sec:probabilistic_properties}
\EDIT{ An important consequence of the \emph{conditional independence} in Equation ~(\ref{eq:conditional_indep}) is that the marginal distributions at aggregate levels $\mathbf{y}_{[a],\tau}$ can be computed via simple component-wise addition of the lower level Poisson rates. Consider an aggregate level $y_{\alpha, \tau} = y_{\beta_1, \tau} + y_{\beta_2, \tau}$. The marginal distribution for $y_{\alpha, \tau}$ can be derived from the joint distribution in Equation~(\ref{eq:joint_distribution}) as follows. First marginalize all other series and time indices (as done in Section \ref{sec:bottom_marginal_distribution} above), which gives us the joint distribution for $y_{\beta_1, \tau}$ and $y_{\beta_2, \tau}$

\begin{equation*}
    \mathrm{P}(y_{\beta_1, \tau}, y_{\beta_2, \tau}) = \sum_{\kappa=1}^{N_{k}} w_\kappa \; \mathrm{Poisson}(y_{\beta_1,\tau} \vert \lambda_{\beta_1,\kappa,\tau}) \times \mathrm{Poisson}(y_{\beta_2,\tau} \vert \lambda_{\beta_2,\kappa,\tau})
\end{equation*}

Now, the aggregate marginal distribution is 
\begin{eqnarray*}
    \mathrm{P}(y_{\alpha, \tau}) &=& \sum_{y_{\beta_1, \tau}, y_{\beta_2, \tau}} \mathrm{P}(y_{\beta_1, \tau}, y_{\beta_2, \tau}) \; \mathbbm{1}(y_{a,\tau}=y_{\beta_1, \tau} + y_{\beta_2, \tau})   
    %\\
    %            &=& \sum_{\kappa=1}^{N_{k}} w_\kappa \sum_{y_{\beta_1, \tau}, y_{\beta_2, \tau}} \mathrm{Poisson}(y_{\beta_1,\tau} \vert \lambda_{\beta_1,\kappa,\tau}) \; \mathrm{Poisson}(y_{\beta_2,\tau} \vert \lambda_{\beta_2,\kappa,\tau}) \times \\
    %            && \quad \mathbbm{1} (y_{a,\tau}=y_{\beta_1, \tau} + y_{\beta_2, \tau})
\end{eqnarray*}
For each mixture component $\kappa$, the distributions of $y_{\beta_1, \tau}$ and $y_{\beta_2, \tau}$ conditioned on respective Poisson rates $\lambda_{\beta_1, \kappa, \tau}$ and $\lambda_{\beta_2, \kappa, \tau}$ are independent Poisson distributions, and therefore, the distribution of the aggregate is another Poisson distribution with $\lambda_{a,\kappa, \tau} = \lambda_{\beta_1, \kappa, \tau} + \lambda_{\beta_2, \kappa, \tau}$.
\begin{equation*}
    \mathrm{P}(y_{\alpha, \tau}) =  \sum_{\kappa=1}^{N_{k}} w_\kappa \mathrm{Poisson}(y_{a,\tau} \vert \lambda_{a,\kappa, \tau} = \lambda_{\beta_1, \kappa, \tau} + \lambda_{\beta_2, \kappa, \tau})
\end{equation*}

The aggregation rule can be concisely describe as $\blambda_{[a][k],\tau} = \mathbf{A}_{\mathrm{[a][b]}}\blambda_{[b][k], \tau}$ with $\mathbf{A}_{\mathrm{[a][b]}}$ the hierarchical summation matrix defined in Section~\ref{section:hierarchical_forecasting_notation}.} Then for any aggregate level $\alpha \in [a]$ and time $\tau \in [t+1:t+h]$, the marginal distribution is:
\begin{equation}
    \mathrm{P}(y_{\alpha, \tau}) = \sum_{\kappa=1}^{N_k} w_\kappa \mathrm{Poisson}(y_{a,\tau} \vert \lambda_{a,\kappa, \tau})
\end{equation}
The predictive distributions are hierarchically coherent by construction. \EDITtwo{We offer a formal proof of \ours' satisfaction of the probabilistic coherence property from Definition~\ref{def:probabilistic_coherence} in \ref{sec:probabilistic_coherence}.}

\subsection{Covariance Matrix}
Using the law of total covariance and the conditional independence in Equation~(\ref{eq:conditional_indep}), the covariance of any two bottom level series naturally follows (derivation in \ref{appen:correlation}):
\begin{equation}\label{eq:covariance}
    \mathrm{Cov}(y_{\beta, \tau}, y_{\beta', \tau'}) = \sum_{\kappa=1}^{N_k} w_\kappa \left(\lambda_{\beta,\kappa,\tau} - \overline{\lambda}_{\beta,\tau}\right) \left( \lambda_{\beta',\kappa,\tau'} - \overline{\lambda}_{\beta',\tau'}\right)
\end{equation}
for all $\; (\beta, \tau), (\beta', \tau') \in [b][t+1:t+h]$ and $\overline{\lambda}_{\beta,\tau} = \sum_{\kappa\in[k]}w_\kappa \lambda_{\beta, \kappa, \tau}$.


==> sections/section5_discussion.tex <==



==> sections/section6_1_benchmarks.tex <==
\subsection{Hierarchical Forecasting Benchmarks}

We compare against the next forecasting methods. \NaiveBU \ produces univariate bottom-level time series forecasts independently and then sums them according to the hierarchical constraints, a distribution is generated using Gaussian assumptions on the errors. \MinT~\citep{wickramasuriya2019hierarchical_mint_reconciliation} \ that reconciles unbiased independent forecasts and minimizes the variance of the forecast errors. \ERM~\citep{taieb2019hierarchical_regularized_regression} that improves on the unbiasedness assumption of the base forecasts in \MinT \ and aims to minimize the bias-variance trade-off of the forecast errors. The benchmark methods \footnote{The implementation of the models and experiments on hierarchical forecasting applications will be available in the future as an extension to the  \href{https://github.com/awslabs/gluon-ts}{\textcolor{blue}{GluonTS library}}.} are implemented or compiled in the \GluonTS \ library \citep{alexandrov2020package_gluonts}. The original implementation of \MinT \ is available in the R package \hts ~\citep{hyndman2020package_hts}, it has an automatic selection of hyperparameters for the \ARIMA \ and \ETS \ univariate base forecast methods \citep{hyndman2008automatic_arima}.

==> sections/section6_1_data.tex <==
% \subsection{Hierarchical Forecasting Datasets}

% \textcolor{blue}{Fancy introduction to hierarchical forecasting datasets}

% \textbf{Australian Tourism.}

% This detailed Australian Tourism Dataset comes from the National Visitor Survey, managed by the Tourism Research Australia, it is composed of 555 monthly series from 1998 to 2016, it is organized geographically, and purpose of travel. The natural geographical hierarchy comprises seven states, divided further in 27 zones and 76 regions. The purpose of travel categories are holiday, visiting friends and relatives (VFR), business and other. The MinT (Wickramasuriya et al., 2019), among other hierarchical forecasting studies has used the dataset it in the past. \footnote{The \TourismL \ dataset can be publicly accessed in this \href{https://robjhyndman.com/publications/mint/}{\textcolor{blue}{https url}}.}

% \textbf{Australian Tourism.} We use two datasets of Australian Tourism. The first, \Tourism \ ~\citep{canberra2005tourism} is composed of 89 quarterly series from 1998 to 2006, organized geographically, several studies reference this dataset \citep{athanasopoulos2009hierarchical_tourism, hyndman2011optimal_combination_hierarchical}. The second, \TourismL \ ~\citep{wickramasuriya2019hierarchical_mint_reconciliation, canberra2019tourism}, is a detailed version of \dataset{Tourism}, it is composed of 555 quarterly series, organized by geography and purpose-of-travel.


% \begin{figure}[tb]
% \centering
% \includegraphics[width=0.85\linewidth]{images/TourismL_hier_linked_series.pdf}
% \caption{Example of a hierarchically linked time series from the \TourismL \ dataset. The top row shows the total number of tourist visits in Australia, the second row shows the touristic visits with holiday purpose, the third row shows the holiday visits in the state of New South Wales, the fourth row shows the holiday visits in the metropolitan zone of New South Wales, the final row shows the holiday visits to Sidney.} \label{fig:tourisml_data}
% \end{figure}

% \textbf{Australian Labour.} \textcolor{blue}{Encontrar monthly} \Labour \ ~\citep{abs2021australian_labour_dataset} is a summary of the labour force survey data curated by the Australian Bureau of Statistics, it reports the number of employed persons in each ANZCO occupation unit group \citep{abs2021australian_labour_anzco} of main job, by sex, state and territory quarterly from 1986 to 2021. The hierarchy that we consider is defined by \textcolor{red}{359} occupation unit groups, \textcolor{red}{97} minor groups, \textcolor{red}{8} major groups and the total, comprising \textcolor{red}{508 time series}, each with 140 observations.

% \textbf{Australian Tourism.} We use two datasets of Australian Tourism. The first, \Tourism \ ~\citep{canberra2005tourism} is composed of 89 quarterly series from 1998 to 2006, organized geographically, several studies reference this dataset \citep{athanasopoulos2009hierarchical_tourism, hyndman2011optimal_combination_hierarchical}. The second, \TourismL \ ~\citep{wickramasuriya2019hierarchical_mint_reconciliation, canberra2019tourism}, is a detailed version of \dataset{Tourism}, it is composed of 555 quarterly series, organized by geography and purpose-of-travel.

% \textbf{Favorita}: The 2018 Kaggle competition was organized by Corporación Favorita, a major Ecuatorian grocery retailer. \Favorita \ ~\citep{favorita2018favorita_dataset} is comprised of item sales history and promotions information, with additional information of items and stores, regional and national holidays, among other. The task consisted on forecasting sixteen days for the log-sales of each item store combination, for a total of 135K series.

% \textbf{M5 Competition.} The \Mfive \ ~\citep{makridakis2020m5competition_results} dataset was provided in the 2020 competition organized by the Makridakis Open Forecasting Center from the University of Nicosia, and hosted in Kaggle \citep{nicosia2020m5_dataset}. The main task consisted in providing hierarchical point and probabilistic predictions for 28 days ahead for 42840 hierarchically organized sales of Walmart stores in three US States (California, Texas, and Wisconsin). The dataset is organized at the item, department, product and store level details. Additionally it contains temporal covariates like price, promotions, events and calendar variables.

==> sections/section8_acknowledgements.tex <==
Thanks to Dr. Kari Torkkola and Dr. Michael Mahoney for in-depth suggestions and discussion on the presentation and the experiment design. Thanks to all Amazon Forecasting Science team members for their comments and feedback on literature review and writing. Thanks to Stefania La Vattiata and Ricardo Morales for their assistance in the upbeat exposition of the \ourscomplete. The authors are also grateful to Syama Rangapuram and Pedro Mercado that carefully chose and organized hierarchical forecasting baselines. And Federico Garza for his help in the replication of the baselines.


==> tables/crps_results.tex <==
\begin{table*}[tp]
\tiny
%\scriptsize
%\footnotesize
\centering
\caption{Empirical evaluation of probabilistic, hierarchical forecasts. Mean \emph{continuous ranked probability score} (CRPS) for predictions, averaged over 8 runs, at each aggregation level, the best result is highlighted (lower is better). The mean hierarchical methods have unique solutions, and constant results over the runs. \\ 
% \EDIT{\HierEtoE \ and \PERMBU \ produces probabilistically coherent distributional forecasts while the remaining ARIMA based models are not, as they are producing point forecasts satisfying aggregation constraints. In this table, we are currently evaluating CRPS by assuming that the point forecast methods produce degenerate distributional forecast with support at the mean forecast only; we did this for our own proof of concept as the most naive baseline.}
%For IJF submission, we will move the point forecast method results from this table that contains CRPS results, to a new table in the appendix, for comparing forecast accuracy of means against probabilistically coherent models.)\\
\tiny{\textsuperscript{*} The \ARIMA-\ERM \ results for \TourismL \ differ from \cite{rangapuram2021hierarchical_e2e}, as we improved the numerical stability of their implementation.\\
\tiny{\textsuperscript{**} 
\PERMBU-\MinT \ on \TourismL \ is unavailable because the original implementation can't be applied to grouping structures with more than a single hierarchy.
}
}
}
\label{table:empirical_evaluation}
\begin{tabular}{cc|ccccccc}
\toprule
\textsc{Dataset} 
& \textsc{Level} & \thead{\ours-\GroupBU \\ (prob.)} & \thead{\ours-\NaiveBU \\ (prob.)}     & \thead{\HierEtoE \\ (prob.)}                         & \thead{\PERMBU-\MinT\textsuperscript{**} \\ (prob.)} & \thead{\ERM\textsuperscript{*} \\ (mean)} & \thead{\MinT-\SHR \\ (mean)} & \thead{\NaiveBU \\ (mean)} \\
\midrule
\multirow{4}{*}{\Traffic}   
 & Overall       & \EDIT{$0.0453 \pm 0.0012$}   & $\mathbf{0.0352 \pm 0.0007}$    & $0.0376 \pm 0.0060$           & $0.0677 \pm 0.0061$           & 0.0466             & 0.077    & 0.0753 \\
 & 1 (geo.)      & \EDIT{$0.0199 \pm 0.0022$}   & $\mathbf{0.0067 \pm 0.0011}$    & $0.0184 \pm 0.0091$           & $0.0331 \pm 0.0085$           & 0.0087             & 0.045    & 0.0363 \\
 & 2 (geo.)      & \EDIT{$0.0269 \pm 0.0012$}   & $0.0145 \pm 0.0008 $            & $0.0181 \pm 0.0086$           & $0.0341 \pm 0.0081$           & $\mathbf{0.0112}$  & 0.046    & 0.0363 \\
 & 3 (geo.)      & \EDIT{$0.0269 \pm 0.0011$}   & $\mathbf{0.0145 \pm 0.0006}$    & $0.0223 \pm 0.0072$           & $0.0417 \pm 0.0061$           & 0.0255             & 0.046    & 0.0453 \\
 & 4 (geo.)      & \EDIT{$0.1078 \pm 0.0011$}   & $0.1050 \pm 0.0004$             & $\mathbf{0.0914 \pm 0.0024}$  & $0.1621 \pm 0.0027$           & 0.1410             & 0.1701   & 0.1832 \\
\midrule
\multirow{8}{*}{\TourismL}
& Overall        & $\mathbf{0.1300 \pm 0.0060}$ & $0.1518 \pm 0.0055$             & $0.1520 \pm 0.0032$           & -                             & 0.1689             & 0.1609.  & 0.1741 \\
& 1 (geo.)       & $\mathbf{0.0557 \pm 0.0113}$ & $0.1043 \pm 0.0144$             & $0.0810 \pm 0.0053$           & -                             & 0.0725             & 0.0438.  & 0.0827 \\
& 2 (geo.)       & $\mathbf{0.0700 \pm 0.0084}$ & $0.1101 \pm 0.0121$             & $0.1030 \pm 0.0030$           & -                             & 0.1071             & 0.0816.  & 0.1035 \\
& 3 (geo.)       & $\mathbf{0.1141 \pm 0.0069}$ & $0.1360 \pm 0.0092$             & $0.1361 \pm 0.0024$           & -                             & 0.1541             & 0.1433.  & 0.1586 \\
& 4 (geo.)       & $\mathbf{0.1570 \pm 0.0057}$ & $0.1669 \pm 0.0085$             & $0.1752 \pm 0.0026$           & -                             & 0.2052             & 0.2036.  & 0.2131 \\
& 5 (prp.)       & $\mathbf{0.0804 \pm 0.0047}$ & $0.1377 \pm 0.0048$             & $0.1027 \pm 0.0062$           & -                             & 0.1095             & 0.0830.  & 0.1002 \\
& 6 (prp.)       & $\mathbf{0.1129 \pm 0.0044}$ & $0.1384 \pm 0.0041$             & $0.1403 \pm 0.0047$           & -                             & 0.1628             & 0.1479.  & 0.1567 \\
& 7 (prp.)       & $0.1901 \pm 0.0051$          & $\mathbf{0.1893 \pm 0.0030}$    & $0.2050 \pm 0.0028$           & -                             & 0.2435             & 0.2437.  & 0.2489 \\
& 8 (prp.)       & $0.2598 \pm 0.0042$          & $\mathbf{0.2414 \pm 0.0018}$    & $0.2727 \pm 0.0017$           & -                             & 0.3076             & 0.3406.  & 0.3379 \\
\midrule
\multirow{4}{*}{\Favorita}  
& Overall        & $\mathbf{0.2010 \pm 0.0091}$ & $0.2651 \pm 0.0060$             & $0.2698 \pm 0.0031$           & $0.2335 \pm 0.0024$           & 0.3675             & 0.2606   & 0.2652 \\
& 1 (geo.)       & $0.1380 \pm 0.0074$          & $0.2083 \pm 0.0098$             & $0.2396 \pm 0.0034$           & $\mathbf{0.1346 \pm 0.0019}$  & 0.2979             & 0.1468   & 0.1556 \\
& 2 (geo.)       & $0.1933 \pm 0.0104$          & $0.2564 \pm 0.0054$             & $0.2664 \pm 0.0031$           & $\mathbf{0.1912 \pm 0.0023}$  & 0.3593             & 0.2176   & 0.2176 \\
& 3 (geo.)       & $\mathbf{0.2034 \pm 0.0103}$ & {$0.2659 \pm 0.0057$}           & $0.2738 \pm 0.0039$           & $0.3419 \pm 0.0027$           & 0.3729             & 0.3769   & 0.3769 \\
& 4 (geo.)       & $\mathbf{0.2693 \pm 0.0013}$ & {$0.3297 \pm 0.0075$}           & $0.3086 \pm 0.0034$           & $0.2766 \pm 0.0029$           & 0.4408             & 0.3096   & 0.3132 \\
\bottomrule
\end{tabular}
\end{table*}
